Coalitional Games in MISO Interference Channels: Epsilon-Core and Coalition Structure Stable Set

The multiple-input single-output interference channel is considered. Each transmitter is assumed to know the channels between itself and all receivers perfectly and the receivers are assumed to treat interference as additive noise. In this setting, noncooperative transmission does not take into account the interference generated at other receivers which generally leads to inefficient performance of the links. To improve this situation, we study cooperation between the links using coalitional games. The players (links) in a coalition either perform zero forcing transmission or Wiener filter precoding to each other. The $\epsilon$-core is a solution concept for coalitional games which takes into account the overhead required in coalition deviation. We provide necessary and sufficient conditions for the strong and weak $\epsilon$-core of our coalitional game not to be empty with zero forcing transmission. Since, the $\epsilon$-core only considers the possibility of joint cooperation of all links, we study coalitional games in partition form in which several distinct coalitions can form. We propose a polynomial time distributed coalition formation algorithm based on coalition merging and prove that its solution lies in the coalition structure stable set of our coalition formation game. Simulation results reveal the cooperation gains for different coalition formation complexities and deviation overhead models.

==> sections/bio.tex <==
\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/mocha}}]{Rami Mochaourab} (S'07--M'13) received the Diplom-Ingenieur (M.Sc.) degree in information systems engineering and Doktor-Ingenieur (Ph.D.) degree in electrical engineering from the Dresden University of Technology, Dresden, Germany, in 2008 and 2012, respectively. From August 2012 until February 2014, he was with Fraunhofer Heinrich-Hertz-Institut Berlin in the Wireless Communications and Networks Department. Currently, he is a postdoctoral research associate with ACCESS Linnaeus Centre, Signal Processing Department, KTH Royal Institute of Technology, Sweden. His research interests are within the fields of resource allocation, signal processing, and game theory for multiuser wireless communication networks. 

Dr. Mochaourab received a Best Student Paper Award at 2011 IEEE International Workshop on Computational Advances in Multi-Sensor Adaptive Processing (CAMSAP) and a Best Paper Award at 2013 IEEE Vehicular Technology Conference (VTC-Spring).
\end{biography}

\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/jorsw}}]{Eduard A. Jorswieck} (S'01--M'05--SM'08) received his Diplom-Ingenieur (M.S.) degree and Doktor-Ingenieur (Ph.D.) degree, both in electrical engineering and computer science from the Technische Universität Berlin, Germany, in 2000 and 2004, respectively. He was with the Fraunhofer Institute for Telecommunications, Heinrich-Hertz-Institut (HHI) Berlin, in the Broadband Mobile Communication Networks Department from December 2000 to February 2008. From April 2005 until February 2008, he was a lecturer at the Technische Universität Berlin. From February 2006 until February 2008, he worked for the Department of Signals, Sensors and Systems at the Royal Institute of Technology (KTH) as a post-doc and Assistant Professor. Since February 2008, he has been the head of the Chair of Communications Theory and Full Professor at Dresden University of Technology (TUD), Germany. He is principal investigator in the excellence cluster center for Advancing Electronics Dresden (cfAED) and founding member of the 5G lab Germany (5Glab.de). His research interests are in the area of signal processing for communications and networks, applied information theory, and communications theory. He has published more than 65 journal papers and some 190 conference papers on these topics. Since 2011, he acts as Associate Editor for IEEE Transactions on Signal Processing. Since 2008, continuing until 2011, he has served as an Associate Editor for IEEE Signal Processing Letters and from 2011 until 2013 as Senior Associate Editor for IEEE Signal Processing Letter. Since 2013, he serves as Associate Editor for IEEE Transactions on Wireless Communications. In 2006, he received the IEEE Signal Processing Society Best Paper Award.
\end{biography}

